Setting the Right Expectations: Algorithmic Recourse Over Time

Algorithmic systems are often called upon to assist in high-stakes decision making. In light of this, algorithmic recourse, the principle wherein individuals should be able to take action against an undesirable outcome made by an algorithmic system, is receiving growing attention. The bulk of the literature on algorithmic recourse to-date focuses primarily on how to provide recourse to a single individual, overlooking a critical element: the effects of a continuously changing context. Disregarding these effects on recourse is a significant oversight, since, in almost all cases, recourse consists of an individual making a first, unfavorable attempt, and then being given an opportunity to make one or several attempts at a later date - when the context might have changed. This can create false expectations, as initial recourse recommendations may become less reliable over time due to model drift and competition for access to the favorable outcome between individuals. In this work we propose an agent-based simulation framework for studying the effects of a continuously changing environment on algorithmic recourse. In particular, we identify two main effects that can alter the reliability of recourse for individuals represented by the agents: (1) competition with other agents acting upon recourse, and (2) competition with new agents entering the environment. Our findings highlight that only a small set of specific parameterizations result in algorithmic recourse that is reliable for agents over time. Consequently, we argue that substantial additional work is needed to understand recourse reliability over time, and to develop recourse methods that reward agents' effort.

==> deprecated.tex <==
    The implementation of consumer-facing Machine Learning (ML) models is becoming increasingly common for high-stakes decision making. This trend motivated the development of Algorithmic Recourse (AR) systems, which provides agents with actionable recommendations to modify adverse outcomes. The majority of AR research focuses on optimizing the recommendations provided in different settings, such as high dimensionality, black-box decision models, causal-based counterfactuals and group-based counterfactuals. Simultaneously, research on the reliability of AR in competitive multi-agent environments is essential to provide trustworthy recourse to all agents, although sparse. Existing literature is also hampered by a set of limitations: closed environments with unlimited resources, limited environment setups, agents with full flexibility for corrective action and lack metrics to analyze these environments. We present an open environment with different types of corrective adaptation behaviors and performance metrics, to better understand and simulate multi-agent AR (MAAR) environments along multiple time-steps. Our contribution is three-fold: (1) understand how different settings of a multi-agent scenario impact the ability of an agent to take successful and reliable AR, (2) a comprehensive set of metrics to monitor ongoing agents' dynamics and (3) demonstrate how these dynamics can be predicted for subsequent time-steps. We define success criteria for MAAR, as well as metrics to quantify and monitor its effectiveness, describe the different parameters used to define the environment, run multiple AR simulations under different conditions to capture the populations' behavior, and propose an approach to estimate the population's expected behavior in following time steps. We found that \hl{...}. 
We expect this work to assist and inform stakeholders in the implementation of reliable AR systems in practical applications.  

==> unused.tex <==
\smallskip
\noindent \textbf{Simulation algorithm.} The algorithm for running our simulation (depicted in Figure~\ref{fig:framework}) takes as an input a black box classifier $f: \mathcal{X} \rightarrow [0,1]$ and a resource constraint $k$ (which we assume, for ease of exposition, to be fixed), and a function for recourse that describes both \emph{adaptation} and \emph{effort} (defined in Section~\ref{sec:problem:simulation}) $a: \mathcal{X} \times \mathcal{X} \rightarrow \mathcal{X} $. It also takes as inputs the parameters in Table~\ref{tab:parameters}. It then executes multiple runs $t_0, \ldots, t_T$ of the multi-agent recourse problem described in Definition~\ref{def:multi-rec}. What follows is a step-by-step description of an execution of the algorithm:

\begin{enumerate}
    \item At time $t=0$, an initial population $P_0$ enters the environment. The score $S_0$ is computed for each agent in $P_0$, and the agents are sorted from highest to lowest by this score. The agents with the top $k$ scores receive a positive outcome (and will later be removed from the environment). The threshold for a positive outcome $s_0$ is set as the minimum score among those agents that in the top $k$. Each agent that received a negative outcome is given a recourse recommendation. We call this population $L_0$. Then, agents will ``react'' to their recommendations according to the function $a$ (which may include applying no changes at all) to form $A_1$. Afterwards, the following process is executed at each time step:
    \item New agents $N_t$ enter the environment, and their scores are computed. At this point, the population $P_t$ of agents is the union of $N_t$ and $A_t$ (the agents that received a negative outcome at the previous time step).
    \item The agents in population $P_t$ are sorted by score. The agents with the top $k$ scores, $P^k_t$, receive the positive outcome. The new threshold, $s_t$, is determined using the score of the lowest-scoring agent in $P^k_t$. The remaining agents $L_t$, receive a recourse recommendation, $R_t$, and take recourse action according to $a(x_t, x_t')$. %, to attempt receiving a positive outcome in the following time step.
    \item From the agents in $L_t$, we create $A_{t+1}$, which is the population of agents after making changes according to the function $a$ and their recourse recommendation.
    \item All agents except those who received a positive outcome (the agents in $P^k_t$) move on to the next time step. %, whereas the winning agents exit the system.
    
\end{enumerate}
%The main steps are summarized in figure \ref{fig:framework}:
%\begin{enumerate}
    % Input A_{t-1}, N_t
    % compute starting population P_{t} = A_{t_1} \cap N_t
%    \item[A] $P_t$ are agents competing at time $t$, as union of adapted users and new users.
    % evaluate every agent by f(x)
%    \item[B] Agents ask for the loan and receives a score from the black-box classifier $f(\cdot)$;
    % compute $s$, select W = top-$k$
%    \item[C-D] $P_t^{k}$ agents get the loan and exit from the game, while the $y_t$ threshold is updated.
    %In this stage, depending on the configuration, some users that adapt to the recourse suggested at $t-1$ may not be selected.
    % generate recourse feedback for L = P \setminus top-$k$
%    \item[E] $P_t \setminus P_t^{k}$ agents receive a recourse feedback %by $r(\cdot)$;
    % adapt L
%    \item[F] Each agent $x_t$ that received a recourse feedback $x'$ adapts to a new configuration $a(x^t,x') = x^{t+1}$, that is the configuration of the agent at $t+1$;
    % return a(L) as A
%    \item[G] $N_t$ new agents are added in the game and everything start again.
%\end{enumerate}

\renewcommand{\algorithmicrequire}{\textbf{Inputs:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}

\begin{algorithm}[thb]
    \caption{Simulating multi-agent recourse over time}
    \label{alg:rec}
    \begin{algorithmic}[1]
    \Require Classifier $f:\mathcal{X} \rightarrow [0,1]$; function for generating recourse recommendations $r:\mathcal{X} \rightarrow \mathcal{X}$,  function describing agent recourse actions $a:\mathcal{X} \times \mathcal{X} \rightarrow \mathcal{X}$,(with $l$ and $g$); number of time steps $T$, $k$ number of favorable outcomes per time step, initial population size $|P_0|$, number of new agents at each time step $|N_t|$; a number of time steps $T$.
    \Ensure The sequence of sets of agents $\{P_{t_0}, \dots, P_{t_T}\}$ in their final state for each time step.
    
    \State $t \gets 0$
    \State $P_0 \gets $ set of initial population of agents enter the environment%$n_o \in \mathcal{N}^+$ agents
    \While{$t<T$}
        \If{$t \neq 0$}
            \State $N_t \gets$ set of new agents entering the environment;
            \State $P_t \gets A_t \cup N_t$, join sets to create full population; \hfill\Circled{A} \Circled{H}
        \EndIf
        
        \State $S_t \gets \{f(x_t) | \forall x_t \in P_t, f(x_t)\}$, compute score; \hfill\Circled{B}
        \State $\bar{P}_t \gets sort(P_t,S_t)$, sorts agents by score; \hfill\Circled{C}
        \State $P^k_t \gets select\_top\_k(\bar{P}_t)$, select agents w/ pos. outcome (\ie the top-$k$ agents); \hfill\Circled{D}
        \State $s_t \gets update(P^k_t)$, update the decision threshold to be the minimum score from $P^k_t$d; \hfill\Circled{E}
        \State $L_t \gets P_t \setminus P^k_t$, select agents w/ neg. outcome;
        \State $R_t \gets \{x'| \forall x_t \in L_t, r(x_t)=x'\}$, generate recourse recommendations; \hfill\Circled{F}
        \State $A_{t+1} \gets \{x_{t+1}| \forall x_t \in L_t, a(x_t,x') = x_{t+1}\}$, take action and create set of agents that move to the next time-step \hfill\Circled{G}
        %\State $N_{t+1} \gets $ select $n_{t+1} \in \mathcal{N}^+$ new agents; \hfill\Circled{H}
        \State $t \gets t + 1$
    \EndWhile
    \end{algorithmic}
\end{algorithm}
